Convex Optimization for Trajectory Generation

Reliable and efficient trajectory generation methods are a fundamental need for autonomous dynamical systems of tomorrow. The goal of this article is to provide a comprehensive tutorial of three major convex optimization-based trajectory generation methods: lossless convexification (LCvx), and two sequential convex programming algorithms known as SCvx and GuSTO. In this article, trajectory generation is the computation of a dynamically feasible state and control signal that satisfies a set of constraints while optimizing key mission objectives. The trajectory generation problem is almost always nonconvex, which typically means that it is not readily amenable to efficient and reliable solution onboard an autonomous vehicle. The three algorithms that we discuss use problem reformulation and a systematic algorithmic strategy to nonetheless solve nonconvex trajectory generation tasks through the use of a convex optimizer. The theoretical guarantees and computational speed offered by convex optimization have made the algorithms popular in both research and industry circles. To date, the list of applications includes rocket landing, spacecraft hypersonic reentry, spacecraft rendezvous and docking, aerial motion planning for fixed-wing and quadrotor vehicles, robot motion planning, and more. Among these applications are high-profile rocket flights conducted by organizations like NASA, Masten Space Systems, SpaceX, and Blue Origin. This article aims to give the reader the tools and understanding necessary to work with each algorithm, and to know what each method can and cannot do. A publicly available source code repository supports the provided numerical examples. By the end of the article, the reader should be ready to use the methods, to extend them, and to contribute to their many exciting modern applications.

==> latex_common/optimization.tex <==
\ExplSyntaxOn
\makeatletter

\def\objective@label{objective}

\tl_new:N \l_opti_task_tl
\tl_new:N \l_opti_label_tl
\tl_new:N \l_opti_vars_tl
\tl_new:N \l_opti_objective_tl
\tl_new:N \l_opti_result_tl

\define@key{optim@keys}{task}{\tl_set:Nn \l_opti_task_tl {#1}}
\define@key{optim@keys}{label}{\tl_set:Nn \l_opti_label_tl {#1}}
\define@key{optim@keys}{variables}{\tl_set:Nn \l_opti_vars_tl {#1}}
\define@key{optim@keys}{objective}{\tl_set:Nn \l_opti_objective_tl {#1}}
\define@key{optim@keys}{result}{\tl_set:Nn \l_opti_result_tl {#1}}

\newenvironment{optimization}[1][]{
  \setkeys{optim@keys}{task=\min,#1}
  \setkeys{optim@keys}{label=,#1}
  \setkeys{optim@keys}{variables=,#1}
  \setkeys{optim@keys}{objective=,#1}
  \subequations
  \label{problem:\tl_use:N \l_opti_label_tl}
  \align
  \optilabel{\objective@label}
  \ifthenelse{\equal{\tl_use:N \l_opti_result_tl}{}}{}{%
    \tl_use:N \l_opti_result_tl =}%
  \tl_use:N \l_opti_task_tl\c_math_subscript_token
  {\mathclap{\tl_use:N \l_opti_vars_tl}}\textnormal{\ }
  & \tl_use:N \l_opti_objective_tl \\
  \mrm[t]{s.t.}\textnormal{\ }
}{
  \endalign
  \endsubequations
}

\newenvironment{optimization*}[1][]{
  \setkeys{optim@keys}{task=\min,#1}
  \setkeys{optim@keys}{variables=,#1}
  \setkeys{optim@keys}{objective=,#1}
  \csname align*\endcsname
  \tl_use:N \l_opti_task_tl\c_math_subscript_token
  {\mathclap{\tl_use:N \l_opti_vars_tl}}\textnormal{\ }
  & \tl_use:N \l_opti_objective_tl \\
  \mrm[t]{s.t.}\textnormal{\ }
}{
  \csname endalign*\endcsname
}

\newcommand{\optilabel}[2][eq]{\label{#1:\tl_use:N \l_opti_label_tl _#2}}
\newcommand{\optieqref}[2]{\eqref{eq:#1_#2}}
\newcommand{\optiobjref}[1]{\eqref{eq:#1_\objective@label}}

\makeatother
\ExplSyntaxOff

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> sections/abbreviations.tex <==
\lcvx & Lossless convexification \\
LTV & Linear time-varying \\
SCP & Sequential convex programming \\
SQP & Sequential quadratic programming \\
LP & Linear program \\
QP & Quadratic program \\
SOCP & Second-order cone program \\
SDP & Semidefinite program \\
MILP & Mixed-integer linear program \\
NLP & Nonlinear (nonconvex) program \\
IPM & Interior point method \\
MPC & Model predictive control \\
ISS & International Space Station \\
KKT & Karush-Kuhn-Tucker \\
ODE & Ordinary differential equation \\
ZOH & Zeroth-order hold \\
FOH & First-order hold \\
DoF & Degree of freedom \\
Programming & Optimization

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/front_cover.tex <==
\ifmakeprettycsm
\makeatletter

\tikzset{
  every node/.append style={
    outer sep=0pt,
    inner sep=0pt,
    minimum size=0pt
  }
}

\twocolumn[{\begin{figure}[H]
    \begin{tikzpicture}[%
      overlay,
      remember picture,
      shift={(current page.north east)}]

      \node[anchor=north east] (image) at (0,0)
      {{\includegraphics[page=1]{cover_art}}};

    \end{tikzpicture}
    \vspace{16.5cm}
  \end{figure}}]

\begin{figure*}[t]
  \begin{tikzpicture}[%
    overlay,
    remember picture,
    shift={(current page.north west)}]

    \node[anchor=north west] (image) at (0,0)
    {\includegraphics[page=2]{cover_art}};

  \end{tikzpicture}
  \vspace{15cm}
\end{figure*}

\makeatother
\else
\ifmakearxivcsm
\def\affilspace{1pt}
\def\uwaffil{\hspace{\affilspace}\hyperlink{uwinfo}{$^{\textsf{a}}$}}
\def\stanfordaffil{\hspace{\affilspace}%
  \hyperlink{stanfordinfo}{$^{\textsf{b}}$}}
\def\authoremail{}
\newcommand{\corresp}[1]{$^{,}$%
  \hyperlink{correspauth}{$^{\star}$}
  \gdef\authoremail{#1}}
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{$\star$}\footnotetext{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
\newcommand{\correspfootnote}{\blfootnote{%
    ~\linkdest{correspauth}{Corresponding author}.

    \hspace{2pt}\phantom{$\star$~}%
    \textit{E-mail address:} \href{mailto:\authoremail}{\authoremail}}}

\twocolumn[{\begin{figure}[H]

    \tikzset{
      cover art/.style={
        anchor=north
      },
      title/.style={
        anchor=north,
        font=\bfseries\sffamily\huge,
        yshift=-\csmtopmargin
      },
      subtitle/.style={
        anchor=north,
        font=\itshape\sffamily\large,
        yshift=-3mm
      },
      authorlist/.style={
        anchor=north,
        font=\sffamily,
        yshift=-4mm,
        align=center,
        text width=1\textwidth
      },
      affil info/.style={
        anchor=north,
        yshift=-6mm,
        scale=0.8,
        font=\sffamily
      },
      abstract/.style={
        anchor=north,
        align=left,
        text width=0.95\textwidth,
        font=\sffamily,
        yshift=-12mm,
        scale=0.85
      },
      abstract rule/.style={
        draw=black,
        line width=1pt,
        line cap=round
      }
    }
    \def\abstractruleshift{4mm}

    \pgfdeclarelayer{fg}
    \pgfsetlayers{main,fg}

    \begin{tikzpicture}[%
      overlay,
      remember picture,
      shift={(current page.north)}]

      \begin{pgfonlayer}{fg}
        \node[cover art] at (0, 0) {\includegraphics{cover_art_arxiv}};
      \end{pgfonlayer}

      \node[title] (title) at (0, 0)
      {{\color{white}Convex} Optimization for Trajectory Generation};

      \node[subtitle] (subtitle) at (title.south)%
      {A Tutorial On Generating Dynamically Feasible Trajectories Reliably And
        Efficiently};

      \node[authorlist] (authors) at (subtitle.south)%
      {\scalebox{0.9}{
          \begin{minipage}[c]{1.0\linewidth}
            \centering
            Danylo Malyuta\uwaffil\corresp{danylo@malyuta.name}, %
            Taylor P. Reynolds\uwaffil, %
            Michael Szmuk\uwaffil, %
            Thomas Lew\stanfordaffil, \\%
            Riccardo Bonalli\stanfordaffil, %
            Marco Pavone\stanfordaffil, %
            and \Behcet{} \Acikmese{}\uwaffil
          \end{minipage}
        }};

      \node[affil info] (uw info) at (authors.south)
      {\linkdest{uwinfo}{$^{\textsf{a}}$} %
        William E. Boeing Department of Aeronautics and Astronautics, %
        University of Washington, Seattle, WA 98195, USA};

      \node[affil info,yshift=5mm]
      (stanford info) at (uw info.south)
      {\linkdest{stanfordinfo}{$^{\textsf{b}}$} %
        Department of Aeronautics and Astronautics, %
        Stanford University, Stanford, CA 94305, USA};

      \node[abstract] (abstract) at (stanford info.south)
      {\input{sections/abstract}};

      \draw[abstract rule]
      ($(abstract.north west)+(0,\abstractruleshift)$) --
      ($(abstract.north east)+(0,\abstractruleshift)$);

      \draw[abstract rule]
      ($(abstract.south west)+(0,-\abstractruleshift)$) --
      ($(abstract.south east)+(0,-\abstractruleshift)$);

    \end{tikzpicture}

    \vspace{12cm}

  \end{figure}}]

\correspfootnote
\else
\title{Convex Optimization for Trajectory Generation\\
  \Large A Tutorial On Generating Dynamically Feasible Trajectories
  Reliably And Efficiently}

\author{%
 Danylo Malyuta,~%
 Taylor P. Reynolds,~%
 Michael Szmuk,~%
 Thomas Lew, \\
 Riccardo Bonalli,~%
 Marco Pavone,~%
 and \Behcet{} \Acikmese{} \\
 POC: D.\ Malyuta (danylo@malyuta.name) \\
 \today}

\maketitle
\fi
\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/symbols.tex <==
$M$ & Matrices are capitalized letters \\
$z$ & A scalar or vector variable \\
$\set S$ & Sets are calligraphic capitalized letters \\
$(a,b,c)$ & Concatenation of column or row vectors \\
$e_i$ & Standard $i$-th standard basis vector \\
$I_n\in\real^{n\times n}$ & Identity matrix \\
$v\skew$ & Skew symmetric matrix representation of a cross product \\
$\diag\pare{a,B,\dots}$ & (Block) diagonal matrix from scalars and/or
matrices \\
$\dom f$ & Domain of a function \\
$\grad_x f$ & The gradient vector or Jacobian matrix of $f$ with
respect to $x$ \\
$f[t]$ & Shorthand for a function evaluated at a particular time (e.g.,
$f(t,x(t),u(t))$) \\
%
\iffalse
$\pd^n$ & The set of $n\times n$ symmetric positive definite matrices \\
$\interior{\set X}$ & interior of $\set X$ \\
$\boundary{\set X}$ & boundary of $\set X$ \\
$A\mathcal X$ & $\{Ax:x\in\mathcal X\}$ \\
$\diff{x}{f}$ & partial derivative of function $f$ wrt argument $x$ \\
$f[t]$ & After introducing a function $f(t,x(t),u(t))$, the explicit
listing of arguments is dropped in favor of $f[t]$ \\
$\conehull \{a_1,a_2,a_3\}$ & Conic hull, or positive span, of a set of
vectors, $\sum_{i=1}^3\alpha_i a_i$ where $\alpha_i\ge 0$ \\
$\optimal{x}$ & Optimal value of a variable $x$ \\
$\optimal{f}[t]$ & Optimal value of a function,
i.e. $f(t,\optimal{a}(t),\optimal{b}(t),\optimal{c}(t))$ \\
$f^{(i)}[t]$ & The $i$-th time derivative \\
$f(\tau^-)$ & Left-hand limit, $\lim_{t\uparrow\tau}f(t)$ \\
$f(\tau^+)$ & Right-hand limit, $\lim_{t\downarrow\tau}f(t)$ \\
$\lbdry\mathcal V$ & Lossless part of the boundary i.e. which projects
back to $\mathcal U$ \\
$\image{A}$ & Image of a matrix is its range space, $\{Ax:x\in\real^n\}$ \\
$\nul{A}$ & Nullspace of a matrix, $\{x : Ax=0\}$ \\
$\setcomplement{\set C}$ & Set complement \\
$x_{\mathcal B}$ & A vector represented in the $\mathcal B$ frame \\
$\norm[2^+]{x}$ & The Eucledian norm squared, $x\T x$ \\
$\brak{f}^+$ & Positive part of function $f$ \\
$\grad_x f(\bar x)$ & Gradient of function $f$ evaluated at $x=\bar x$
\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebar.tex <==

\csmprintsymbollist

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebars/discretization.tex <==
\begin{subsidebar}

  \sbfirstword{Suppose} that we have a continuous-time linear time-varying
  dynamical system governed by the ordinary differential
  equation~\optieqref{scp_gen_cvx}{dynamics}. To temporally discretize this
  system, we choose a set of $N$ temporal nodes:
  \begin{equation}
    \label{eq:sidebar_dynamics_times}
    0 = t_1 < t_2 < \cdots < t_N = 1,
  \end{equation}
  which do not need to be evenly spaced. The objective of any discretization
  method is to represent the state trajectory $x(\cdot):[0,1]\to\reals^n$ at
  each of these temporal nodes as a function of the state, control, and
  parameters at the temporal nodes. Mathematically, this transforms the ODE
  \optieqref{scp_gen_cvx}{dynamics} into a linear time-varying difference
  equation.

  There are countless ways to achieve this objective, and~\cite{Malyuta2019b}
  provides a comparative study of several such methods for motion planning
  problems. When choosing a method, it is important to remember that not all
  discretizations perform equally well. Coarse discretization techniques can
  render a convex subproblem infeasible even if the original optimal control
  problem is feasible. Moreover, different discretization methods will change
  the sparsity properties of the resulting convex subproblem, impacting the
  computational requirements for solving each subproblem at stage
  \alglocation{\solveloc} in \figref{scp_loop}.

  In practice, two methods appear to be the most appropriate for SCP-based
  trajectory generation: pseudospectral and interpolating polynomial
  methods. Pseudospectral discretization has gained popularity after its
  original introduction to the optimal control community by
  Vlassenbroeck~\cite{Vlassenbroeck1988,Vlassenbroeck1988b}. This method
  approximates both the state and control trajectories using a basis of
  so-called Lagrange interpolating polynomials, over a non-uniform temporal
  grid defined by the roots of an orthogonal polynomial
  \cite{deboor1973collocation,rao2010survey,ross2012review,Kelly2017}. In
  contrast, interpolating polynomial methods only approximate the control
  signal. This enables the exact solution of the LTV
  system~\optieqref{scp_gen_cvx}{dynamics} over each time interval, yielding an
  ``exact'' discrete-time representation~\cite{SzmukReynolds2018}. Here, exact
  means that the continuous- and discrete-time states match at the temporal
  nodes. A key attribute of interpolating polynomial discretization is that
  upon convergence, an SCP solution satisfying the discretized dynamics
  \eqref{eq:sidebar_dynamics_dt} will exactly satisfy the original nonlinear
  differential equation~\optieqref{scp_gen_cont}{dynamics}.

  As an example, we shall now present a discretization approach from the
  class of interpolating polynomial methods. This method, called first-order
  hold (FOH) interpolation, provides a suitable balance between optimality,
  feasibility, and computation time. We have found it to work well for many
  problems \cite{Malyuta2019b,SzmukReynolds2018,Scharf2017}.

  In FOH, the control signal $u(\cdot):[0,1]\to\reals^m$ is constrained to be
  a continuous and piecewise affine function of time. By defining the inputs
  at the temporal nodes, $\brac{u_k}_{k=1}^N$, the continuous-time signal is
  obtained by linear interpolation inside each time interval $[t_k,t_{k+1}]$:
  \begin{align}
    u(t) &= \frac{t_{k+1}-t}{t_{k+1}-t_k} u_k +
           \frac{t - t_k}{t_{k+1}-t_k} u_{k+1}, \notag \\
    \label{eq:sidebar_control_foh}
         &\definedas \sigm(t) u_k + \sigp(t) u_{k+1}.
  \end{align}

\end{subsidebar}

\begin{subsidebar}

  \noindent The dynamics~\optieqref{scp_gen_cvx}{dynamics} can then be expressed
  for $t\in[t_k,t_{k+1}]$ as:
  \begin{multline}
    \label{eq:sidebar_disc_ct_withU}
    \dot{x}(t) = A(t)x(t) + B(t)\sigma_-(t) u_k +\\%
    B(t)\sigma_+(t)u_{k+1} + F(t) \pk + r(t),
  \end{multline}
  which is again an LTV system, except for the fact that the control is no
  longer a continuous-time function $u(\cdot)$, but instead it is fully
  determined by the two vectors $u_{k},u_{k+1}\in\reals^m$. A standard result
  from linear systems theory is that the unique solution of
  \eqref{eq:sidebar_disc_ct_withU} is given by \cite{Antsaklis2006}:
  \begin{multline}
    \label{eq:sidebar_ltv_solution}
    x(t) = \stm{t,t_k} x(t_k) +%
    \int_{t_k}^{t} \stm{t,\tau}
    \big[ B(\tau)\sigm(\tau) \uk \\%
    + B(\tau)\sigp(\tau) \ukp + F(\tau) \pk +
    r(\tau) \big]
    \sdd\tau,
  \end{multline}
  where $\stm{t,t_k}$ is the state transition matrix that satisfies the
  following matrix differential equation:
  \begin{equation}
    \label{eq:stm_dynamics}
    \stm[\dot]{t,t_k} = A(t)\stm{t,t_k},~\stm{t_k,t_k}=I_n.
  \end{equation}

  By setting $t=t_{k+1}$, \eqref{eq:sidebar_ltv_solution} allows us to write a
  linear time-varying difference equation that updates the discrete-time
  state $x_k=x(t_k)$ to the next discrete-time state $x_{k+1}=x(t_{k+1})$:
  \begin{subequations}
    \label{eq:sidebar_dynamics_integrals}
    \begin{align}
      \label{eq:sidebar_dynamics_dt}
      \xkp &= A_k \xk + B_k^{\scriptscriptstyle -} \uk +
             B_k^{\scriptscriptstyle +} \ukp + F_k p + r_k, \\
      A_k &= \stm{t_{k+1},t_k}, \\
      \label{eq:sidebar_integrals_start}
      B_k^{\scriptscriptstyle -} &= A_k \int_{t_k}^{t_{k+1}}
                                   \stm{\tau,t_k}^{-1} B(\tau)
                                   \sigm(\tau)\sdd\tau, \\
      B_k^+ &= A_k \int_{t_k}^{t_{k+1}} \stm{\tau,t_k}^{-1}
              B(\tau) \sigp(\tau)\sdd\tau, \\
      F_k &= A_k \int_{t_k}^{t_{k+1}} \stm{\tau,t_k}^{-1}
            F(\tau)\sdd\tau, \\
      \label{eq:sidebar_integrals_end}
      r_k &= A_k \int_{t_k}^{t_{k+1}} \stm{\tau,t_k}^{-1}
            r(\tau)\sdd\tau.
    \end{align}
  \end{subequations}

  In implementation, the state transition matrix, the integrals
  \eqref{eq:sidebar_integrals_start}-\eqref{eq:sidebar_integrals_end}, and the
  reference trajectory's state $\bar x(\cdot)$ are computed simultaneously
  over each interval $[t_k,t_{k+1}]$. This procedure is explained in more
  detail in \cite{Malyuta2019b}, and pseudocode can be found
  in~\cite{Reynolds2020}.

  Ultimately, the update equation \eqref{eq:sidebar_dynamics_dt} is used to write
  $N-1$ affine equality constraints for $k=1,\dots,N-1$, which represent the
  discretized dynamic feasibility constraint on the trajectory. Equation
  \optieqref{subproblem_scvx_dt}{dynamics} provides an example embedding of such
  constraints into an optimization problem.

\end{subsidebar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebars/lcvx_glideslope.tex <==
\begin{csmfigure}[%
  position=H,
  caption={A spacecraft planetary landing glideslope cone can be approximated
    as an affine state constraint
    \optieqref{lcvx_o_linstate}{affine_state}. By adding more facets, a cone with
    circular cross\dash sections
    can be approximated to arbitrary precision.},
  label={sidebar_affine_glideslope}]%
  \centering
  \ifmaketwocolcsm
  \includegraphics[width=\columnwidth]{sidebar_affine_glideslope}
  \else
  \includegraphics[width=0.85\columnwidth]{sidebar_affine_glideslope}
  \fi
\end{csmfigure}

\sbfirstword{A} typical planetary landing problem may include a glideslope
constraint to ensure sufficient elevation during approach and to prevent the
spacecraft from colliding with nearby terrain \cite{Acikmese2007}. Letting
$\hat e_3\in\real^3$ represent the local vertical unit vector at the landing
site, the glideslope requirement can be expressed as a convex second-order
cone constraint:
\begin{equation}
  \label{eq:affinestate:glideslope_soc}
  \hat e_3^\transp x \ge \|x\|_2\cos(\gamma_{\mathrm{gs}}),
\end{equation}
where $\gamma_{\mathrm{gs}}\in [0,\pi/2]$ is the glideslope angle, i.e. the
maximum angle that the spacecraft position vector is allowed to make with the
local vertical. As illustrated in \figref{sidebar_affine_glideslope}, we can
approximate \eqref{eq:affinestate:glideslope_soc} as an intersection of four
halfspaces with the following outward normal vectors:
\begin{subequations}
  \label{eq:affinestate:halfspace_normals}
  \begin{alignat}{3}
    {\color{beamerRed}\hat n_1}
    &{\color{beamerRed}\definedas}
    {\color{beamerRed}\begin{bmatrix}
        \cos(\gamma_{\mathrm{gs}}) \\
        0 \\
        -\sin(\gamma_{\mathrm{gs}})
      \end{bmatrix}},~
    {\color{beamerGreen}\hat n_2}
    &&{\color{beamerGreen}\definedas}
    {\color{beamerGreen}\begin{bmatrix}
        0 \\
        \cos(\gamma_{\mathrm{gs}}) \\
        -\sin(\gamma_{\mathrm{gs}})
      \end{bmatrix}}, \\
    {\color{beamerBlue}\hat n_3}
    &{\color{beamerBlue}\definedas}
    {\color{beamerBlue}\begin{bmatrix}
        -\cos(\gamma_{\mathrm{gs}}) \\
        0 \\
        -\sin(\gamma_{\mathrm{gs}})
      \end{bmatrix}},~
    {\color{beamerDarkYellow}\hat n_4}
    &&{\color{beamerDarkYellow}\definedas}
    {\color{beamerDarkYellow}\begin{bmatrix}
        0 \\
        -\cos(\gamma_{\mathrm{gs}}) \\
        -\sin(\gamma_{\mathrm{gs}})
      \end{bmatrix}}.
  \end{alignat}
\end{subequations}

Thus, \eqref{eq:affinestate:glideslope_soc} can be written in the form
\optieqref{lcvx_o_linstate}{affine_state} by setting:
\begin{equation}
  \label{eq:Hh_matrices_affine_glideslope}
  H =
  \begin{bmatrix}
    {\color{beamerRed}\hat n_1}^\transp \\
    {\color{beamerGreen}\hat n_2}^\transp \\
    {\color{beamerBlue}\hat n_3}^\transp \\
    {\color{beamerDarkYellow}\hat n_4}^\transp
  \end{bmatrix},~
  h = 0\in\real^4.
\end{equation}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebars/lcvx_input_cut.tex <==
\begin{csmfigure}[%
  position=H,
  caption={Halfspace constraints from
    \optieqref{lcvx_o_linstate}{affine_input} can be used to select only
    portions of the nonconvex input set defined by
    \optieqref{lcvx_o_linstate}{bounds}. The remaining feasible input set is
    filled in red.},
  label={sidebar_inputcut}]%
  \centering
  \includegraphics[width=0.5\columnwidth]{sidebar_inputcut}
\end{csmfigure}

\sbfirstword{The} input constraint set defined by
\optieqref{lcvx_o_linstate}{bounds} generally lacks the ability to describe
constraints on individual input components, or on combinations thereof. To
enhance the descriptiveness of the input constraint set, halfspace constraints
in \optieqref{lcvx_o_linstate}{affine_input} may be used. This is illustrated
in \figref{sidebar_inputcut} where $g_0(\cdot)=\|\cdot\|_1$,
$g_1(\cdot)=\|\cdot\|_2$, and
\begin{equation}
  C =
  \begin{bmatrix}
    \hat n_1^\transp \\
    \hat n_2^\transp
  \end{bmatrix},~
  c =
  \begin{bmatrix}
    c_1 \\
    0
  \end{bmatrix}.
\end{equation}

For example, $u_1$ and $u_2$ may describe the concentrations of two chemical
reactants -- hydrochloric acid (\ch{HCl}) and ammonia (\ch{NH3}) -- to
produce ammonium chloride (\ch{NH4Cl}). Then, the first affine constraint may
describe the maximum concentration of \ch{NH3} while the second affine
constraint may describe an inter-dependency in the concentrations of both
reactants. Meanwhile, the by-now familiar constraint
\optieqref{lcvx_o_linstate}{bounds} describes the joint reactant concentration
upper and lower bounds.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebars/lcvx_lower_bound.tex <==
\begin{csmfigure}[%
  position=H,
  caption={Relaxation of the nonconvex input constraint set
    \eqref{eq:inputrelax:lb_convexify_1} to the convex set
    \eqref{eq:inputrelax:lb_convexify_2} by using a slack input
    $\sigma$. If the optimal input
    $(\optimal{u},\optimal{\sigma})\in\lbdry\mathcal V$
    \eqref{eq:inputrelax:relaxed_set_lossless_bdry}, then $\optimal{u}$ is
    feasible for the nonconvex constraint
    \eqref{eq:inputrelax:lb_convexify_1}.},
  label={sidebar_input_relaxation}]%
  \centering
  \includegraphics[width=0.95\columnwidth]{sidebar_input_relaxation}
\end{csmfigure}

\sbfirstword{A} typical rocket engine's thrust is upper bounded by the
engine's performance and lower bounded by combustion instability issues for
small thrusts. Thus, \optieqref{lcvx_o_nostate}{bounds} can be written as
\begin{equation}
  \label{eq:inputrelax:lb_convexify_1}
  \rho_{\min}\le\|u\|_2\le\rho_{\max},
\end{equation}
so that $g_0(u)=g_1(u)\definedas\|u\|_2$. The relaxation
\optieqref{lcvx_r_nostate}{bounds}-\optieqref{lcvx_r_nostate}{lcvx_equality}
then becomes:
\begin{equation}
  \label{eq:inputrelax:lb_convexify_2}
  \rho_{\min}\le\sigma,~\|u\|_2\le\min(\sigma,\rho_{\max}).
\end{equation}

\figref{sidebar_input_relaxation} shows how for $u\in\real^2$, going from
\eqref{eq:inputrelax:lb_convexify_1} to \eqref{eq:inputrelax:lb_convexify_2}
lifts a nonconvex annulus to a convex volume $\mathcal V$,
\ifmaketwocolcsm
\begin{multline}
  \label{eq:inputrelax:relaxed_set}
  \mathcal V \definedas \{(u,\sigma)\in\real^{3}:\rho_{\min}\le\sigma, \\
  \|u\|_2\le\min(\sigma,\rho_{\max}) \}.
\end{multline}
\else
\begin{equation}
  \label{eq:inputrelax:relaxed_set}
  \mathcal V \definedas \{(u,\sigma)\in\real^{3}:\rho_{\min}\le\sigma,
  \|u\|_2\le\min(\sigma,\rho_{\max}) \}.
\end{equation}
\fi

The drawback is that inputs that were not feasible for
\eqref{eq:inputrelax:lb_convexify_1} become feasible for
\eqref{eq:inputrelax:lb_convexify_2}. In particular, any $u$ for which
$\|u\|_2<\rho_{\min}$ is now feasible. However, for the special case of
$(u,\sigma)\in\lbdry\mathcal V$, where:
\ifmaketwocolcsm
\begin{multline}
  \label{eq:inputrelax:relaxed_set_lossless_bdry}
  \lbdry\mathcal V\definedas \{(u,\sigma)\in\real^3: \rho_{\min}\le\sigma, \\
  \|u\|_2=\min(\sigma,\rho_{\max})\},
\end{multline}
\else
\begin{equation}
  \label{eq:inputrelax:relaxed_set_lossless_bdry}
  \lbdry\mathcal V\definedas \{(u,\sigma)\in\real^3: \rho_{\min}\le\sigma,
  \|u\|_2=\min(\sigma,\rho_{\max})\},
\end{equation}
\fi
the input $u$ is feasible. The goal of lossless convexification is to show
that this occurs at the global optimum of \pref{lcvx_r_nostate}, in other
words
$(\optimal{u}(t),\optimal{\sigma}(t))\in\lbdry\mathcal V$. \tref{nostate}
guarantees this.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebars/lcvx_max_speed.tex <==
\begin{csmfigure}[%
  position=H,
  caption={Illustration of the boundary of a maximum velocity constraint,
    which can be expressed as \optieqref{lcvx_o_quadstate}{max_speed}.},
  label={sidebar_quad_velocity}]%
  \centering
  \includegraphics[width=0.5\columnwidth]{velocity_constraint}
\end{csmfigure}

\sbfirstword{If} we set $A=I_n$ and $B=I_n$ in \pref{lcvx_o_quadstate} then the
state $x_2$ can be interpreted as a vehicle's velocity. A maximum velocity
constraint $\norm[2]{x_2}\le v_{\max}$ can then be equivalently written in
the form of \optieqref{lcvx_o_quadstate}{max_speed} as
\begin{equation}
  x_2\T (v_{\max}^{-2} I_n)x_2 \le 1.
\end{equation}

\figref{sidebar_quad_velocity} illustrates the maximum velocity constraint.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebars/lcvx_nonlinear.tex <==
\begin{subsidebar}

\begin{csmfigure}[%
  position=H,
  caption={Illustrations of two nonlinear system for which the
    lossless convexification result of \tref{nonlinear} can be applied.}]%
  \centering
  \begin{subfigure}[b]{0.48\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{lcvx_nonlinear_rocket}
    \caption{Landing a rocket in the presence of nonlinear gravity and
      atmospheric drag.}
    \label{fig:lcvx_nonlinear_rocket}
  \end{subfigure}%
  \hfill%
  \begin{subfigure}[b]{0.48\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{lcvx_nonlinear_uav}
    \caption{Autonomous aircraft trajectory generation with a stall
      constraint and aerodynamic drag.}
    \label{fig:lcvx_nonlinear_uav}
  \end{subfigure}
\end{csmfigure}

  \sbfirstword{At} first sight, the discussion around
  \corref{nonlinear_1,nonlinear_2} may be hard to parse into something
  useful. However, we will now show two concrete and very practical examples
  of dynamical systems that satisfy these corollaries. Both examples
  originate from \cite{Blackmore2012}.

  \subsection{Nonlinear Rocket Landing}

  First, \lcvx can be used for rocket landing with nonlinear gravity and
  aerodynamic drag. Both effects are important for landing either on small
  celestial bodies with a weak gravitational pull, or on planets with a thick
  atmosphere (such as our very own Earth). In this case, the lander dynamics
  can be written as:
  \begin{subequations}
    \label{eq:nonlinear_rocket_dynamics}
    \begin{align}
      \label{eq:nonlinear_rocket_dynamics_accel}
      \ddot r(t) &= g(r(t))-\frac{c}{m(t)}\norm[2]{\dot r(t)}\dot r(t)+\frac{T(t)}{m(t)}, \\
      \dot m(t) &= -\alpha\norm[2]{T(t)},
    \end{align}
  \end{subequations}
  where $r$ denotes position, $m$ is mass, $T$ is thrust, $c$ is the drag
  coefficient, $\alpha$ is inversely proportional to the rocket engine's
  specific impulse, and $g:\reals^3\to\reals^3$ is the nonlinear gravity
  model. An illustration is given in \figref{lcvx_nonlinear_rocket}.

  We can rewrite the above dynamics using the template of
  \optieqref{lcvx_o_nonlinear}{dynamics} by defining the state
  $x\definedas (r,\dot r,m)\in\reals^7$, the input
  $u\definedas T\in\reals^3$, and the input penalty function
  $g(u)\definedas\norm[2]{u}$. The equations of motion can then be written as
  (omitting the time argument for concision):
  \begin{align}
    f(t,x,u,g(u))
    &= \Matrix{
      f_{r}(x,u) \\
    f_{\dot r}(x) \\
    f_{m}(g(u))
    }, \nonumber \\
    &= \Matrix{
      \dot r \\
    g(r)-cm\inv\norm[2]{\dot r}\dot r+Tm\inv \\
    -\alpha \norm[2]{T}
    }. \nonumber
  \end{align}

\end{subsidebar}

\begin{subsidebar}

  This system belongs to the class in \corref{nonlinear_2}. In particular, let
  $f_1=(f_r,f_{\dot r})$ and $f_2=f_m$. Working out the algebra in
  \eqref{eq:lcvx_o_nonlinear_class2_M3}, we have:
  \begin{equation}
    M = \Matrix{
      0 & m\inv I \\
      m\inv I & M_{22}},
  \end{equation}
  where
  $M_{22}=-\frac{c}{m^2}\left(\norm[2]{\dot r}I+%
    \frac{\dot r\dot r\T}{\norm[2]{\dot r}}\right)+%
  \alpha\frac{TT\T}{m^2\norm[2]{T}}$. Thanks
  to the off-diagonal terms, $\nul(M)=\{0\}$ unconditionally, so the rocket
  lander dynamics satisfy the requirements of \corref{nonlinear_2}.

  \subsection{AAV Trajectory Generation Without Stalling}

  An autonomous aerial vehicle (AAV) can lose control and fall out of the sky
  if its airspeed drops below a certain value. This occurs because the wings
  fail to generate enough lift, resulting in an aerodynamic \alert{stall}. It
  was shown in \cite{Blackmore2012} that a stall speed constraint of the form
  $v_{\min}\le\norm[2]{v}$ can be handled by \lcvx via the following
  dynamics:
  \begin{subequations}
    \label{eq:uav_dynamics}
    \begin{align}
      \dot r(t) &= v(t)+v_{\infty}(t), \\
      \dot v(t) &= \kappa \bigl(v_d(t)-v(t)\bigr)-c\norm[2]{v(t)}v(t),
    \end{align}
  \end{subequations}
  where $v$ is the airspeed, $\dot r$ is the ground velocity, and $v_{\infty}$
  is the velocity of the air mass relative to the ground (also known as the
  freestream velocity). An illustration is given in
  \figref{lcvx_nonlinear_uav}.

  The key transformation in \eqref{eq:uav_dynamics} is to make the desired
  airspeed $v_d$ the control variable, and to include a velocity control
  inner-loop via a proportional controller with gain $\kappa$. Because the
  velocity dynamics are of first\dash order, $v$ converges to $v_d$ along a
  straight path in the velocity phase plane, hence the stall speed constraint
  is closely approximated for small control errors $\norm[2]{v_d-v}$.

  We can rewrite the dynamics using the template of
  \optieqref{lcvx_o_nonlinear}{dynamics} by defining the state
  $x\definedas (r,v)\in\reals^6$ and the input
  $u\definedas v_d\in\reals^3$. The equations of motions can then be written as:
  \begin{align}
    f(t,x,u,g(u))
    &= \Matrix{
      f_{r}(t,x) \\ f_{v}(x,u)
    }, \nonumber \\
    &= \Matrix{
      v+v_\infty \\ -\kappa v-c\norm[2]{v}v+\kappa v_d
    }. \nonumber
  \end{align}

  This system belongs to the class in \corref{nonlinear_1}. In particular, let
  $f_1=f_r$ and $f_2=f_{v}$. We then have $\grad_u f_2 = -\kappa I$ and
  $\grad_{x_2} f_1 = I$. Therefore, $\nul(\grad_u f_2)=\{0\}$ and
  $\nul(\grad_{x_2} f_1)=\{0\}$, so the aircraft dynamics satisfy the
  requirements of \corref{nonlinear_1}.

\end{subsidebar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebars/lcvx_pointing.tex <==
\begin{csmfigure}[%
  position=H,
  caption={Relaxation of the nonconvex input set
    \eqref{eq:sidebar_pointing_convexify_1} to a convex set
    \eqref{eq:sidebar_pointing_convexify_2} via intersection with a halfspace
    in the lifted $(u,\sigma)$ space. If the optimal input
    $(\optimal{u},\optimal{\sigma})\in\lbdry\mathcal V$ then $\optimal{u}$ is
    feasible for the nonconvex constraint
    \eqref{eq:sidebar_pointing_convexify_1}.},
  label={sidebar_pointing_relaxation}]%
  \centering
  \includegraphics[width=0.95\columnwidth]{sidebar_pointing_relaxation}
\end{csmfigure}

\sbfirstword{Practical} mechanical systems, such as Segways and rockets, may
have a constraint on their tilt angle away from an upright orientation. To
model such cases, the inequality \optieqref{lcvx_o_nostate_pointing}{pointing}
can be specialized to an input pointing constraint. By choosing
$\hat n_g=\cos(\theta_{\max})$ and $g_0(u)=\|u\|_2$, the constraint becomes
\begin{equation}
  \label{eq:sidebar_pointing_convexify_1}
  \hat n_u^\transp u\ge\|u\|_2\cos(\theta_{\max}),
\end{equation}
which constrains $u$ to be no more than $\theta_{\max}$ radians away from a
nominal pointing direction $\hat n_u$. The relaxed constraint
\optieqref{lcvx_r_nostate_pointing}{pointing} becomes
\begin{equation}
  \label{eq:sidebar_pointing_convexify_2}
  \hat n_u^\transp u\ge\sigma\cos(\theta_{\max}),
\end{equation}
which is a halfspace constraint and is thus convex even for
$\theta_{\max}>\pi/2$, when \eqref{eq:sidebar_pointing_convexify_1} becomes
nonconvex.

\figref{sidebar_pointing_relaxation} shows how for $u\in\real^2$, relaxing
\eqref{eq:sidebar_pointing_convexify_1} to
\eqref{eq:sidebar_pointing_convexify_2} lifts an obtuse ``pie slice'' to a
convex halfspace $\mathcal V$,
\begin{equation}
  \label{eq:pointingrelax:relaxed_set}
  \mathcal V \definedas \{(u,\sigma)\in\real^{3}:%
  \hat n_u^\transp u\ge\sigma\cos(\theta_{\max}),~\|u\|_2\le\sigma\}.
\end{equation}

The drawback is that inputs that were not feasible for
\eqref{eq:sidebar_pointing_convexify_1} become feasible for
\eqref{eq:sidebar_pointing_convexify_2}. In particular, low magnitude inputs
for which $\hat n_u^\transp u<\|u\|_2\cos(\theta_{\max})$ become
feasible. However, if $(u,\sigma)\in\lbdry\mathcal V$,
\begin{equation}
  \label{eq:pointingrelax:lbdry_relaxed_set}
  \lbdry\mathcal V \definedas \{(u,\sigma)\in\real^{3}:%
  \hat n_u^\transp u\ge\sigma\cos(\theta_{\max}),~\|u\|_2=\sigma\},
\end{equation}
then the input $u$ satisfies the original constraint
\eqref{eq:sidebar_pointing_convexify_1}. The goal of lossless convexification
is to show that this occurs at the global optimum, in other words
$(u^*,\sigma^*)\in\lbdry\mathcal V$. \tref{nostate_pointing} guarantees this.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebars/lcvx_pointwise_state.tex <==
\begin{csmfigure}[%
  position=H,
  caption={Illustration of when lossless convexification with general convex
    state constraints may fail. The two figures on the right show an in-plane
    projection of the 3D figure on the left. In (a) the glideslope constraint
    is only activated once prior to landing, hence the solution is
    lossless. In (b) the constraint is activated for a non-trivial duration
    and the solution may be infeasible over that interval.},
  label={sidebar_genstate_activation}]%
  \centering
  \includegraphics[width=1\columnwidth]{sidebar_genstate_activation}
\end{csmfigure}

\sbfirstword{Let} us go back to the landing glideslope constraint for a
spacecraft, which was previously motivated in
\sbref{sidebar_affinestate}. Because \pref{lcvx_o_genstate} allows us to use
any convex state constraint, we can directly use the second-order cone
constraint \eqref{eq:affinestate:glideslope_soc}.

As illustrated in \figref{sidebar_genstate_activation}, lossless
convexification in this case will only hold if the spacecraft touches the
``landing cone'' a finite % (in fact, countable)
number of times. In \fakesubfigref{sidebar_genstate_activation}{a}, the glideslope
constraint is activated only once at time $t_1$ prior to landing. Hence,
$\set T=\{t\in [0,t_f]:x(t)\in\boundary{\set X}\}=\{t_1,t_f\}$ is a discrete set
and \tref{genstate} holds. Note that the constraint may be activated at other
times, e.g. $\set T=\{t_1,t_2,t_f\}$, as long as these times are all isolated
points.

In \fakesubfigref{sidebar_genstate_activation}{b} there is an interval of time for which
the glideslope constraint is active. This results in a non-discrete set of
state constraint activation times $\set T=[t_1,t_2]\union \{t_f\}$. For
$t\in[t_1,t_2]$, there is no \lcvx guarantee and the solution of
\pref{lcvx_r_genstate} may be infeasible for \pref{lcvx_o_genstate} over that
interval.

For historical context, \lcvx theory was initially developed specifically for
planetary rocket landing. For this application, glideslope constraint
activation behaves like \fakesubfigref{sidebar_genstate_activation}{a}, so \lcvx holds for
that application. Indeed, the constraint \eqref{eq:affinestate:glideslope_soc}
was part of NASA Jet Propulsion Laboratory's optimization-based rocket
landing algorithm flight tests
\cite{acikmese2013flight,Scharf2014,Scharf2017,flights2012a,flights2012b}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sidebars/lcvx_pwa.tex <==
\begin{subsidebar}

  \sbfirstword{Piecewise} affine functions can be used for arbitrarily
  accurate approximation of any nonlinear function. This is the technique used
  by \cite{Blackmore2012} to write the nonlinear dynamics
  \optieqref{lcvx_r_nonlinear}{dynamics} in piecewise affine form. Doing so
  enables solving \pref{lcvx_r_nonlinear} to global optimality via
  mixed-integer programming, which is imperative for the \lcvx guarantee of
  \tref{nonlinear}. We now show how a piecewise affine approximation can be
  obtained in the general case, and concretely in the case of the dynamics
  from \sbref{lcvx_nonlinear}.

  \subsection{General Case}

  We begin by finding a first\dash order approximation of the nonlinear equation
  $f:\reals\times\reals^n\times\reals^m\times\reals\to\reals^n$ from
  \optieqref{lcvx_r_nonlinear}{dynamics} about an operating point
  $(t,\bar x^i,\bar u^i)\in\reals\times\reals^n\times\reals^m$, where $i$ is an
  integer index that shall become clear in a moment. Without loss of generality,
  assume that $f$ is decomposable into an affine and a non-affine part:
  \begin{equation}
    \label{eq:f_decomposition}
    f=f_a+f_{na}.
  \end{equation}

  The first\dash order Taylor expansion of $f$ is given by:
  \begin{align}
    \nonumber
    f &\approx f_a+f_{na}^i, \\
    \label{eq:pwa_f_linearization}
    f_{na}^i &\definedas \bar f_{na}+
               \bigl(\grad_x \bar f_{na}\bigr)(x-\bar x)+
               \bigl(\tilde\grad_u \bar f_{na}\bigr)(u-\bar u),
  \end{align}
  where we have used the shorthand:
  \begin{subequations}
    \begin{align}
      f_{na}^i &= f_{na}^i(t,x,u,g(u)), \\
      \bar f_{na} &= f_{na}(t,\bar x^i,\bar u^i,g(\bar u^i)), \\
      \label{eq:grad_u_f}
      \tilde\grad_u f_{na} &= \grad_u f_{na}+(\grad_g f_{na})(\grad g)\T.
    \end{align}
  \end{subequations}

  In \eqref{eq:grad_u_f}, we understand $\grad_g f_{na}$ as the Jacobian of
  $f_{na}$ with respect to its fourth argument. Suppose that the linearization
  in \eqref{eq:pwa_f_linearization} is sufficiently accurate only over the
  hyperrectangular region $\set R^i\subset\reals^n\times\reals^m$ defined by the
  following inequalities:
  \begin{subequations}
    \begin{alignat}{3}
      \bar x^i+b_{L,x}^i &\le x &&\le\bar x^i+b_{U,x}^i, \\
      \bar u^i+b_{L,u}^i &\le u &&\le\bar u^i+b_{U,u}^i,
    \end{alignat}
  \end{subequations}
  where $b_{L,x}^i$ and $b_{U,x}^i$ represent the upper and lower bounds on
  the state, while $b_{L,u}^i$ and $b_{U,u}^i$ relate to the input. The index
  $i$ now takes on a clear meaning: it represents the $i$-th ``validity''
  region. Without loss of generality, we assume
  $\set R^i\intersection\set R^j=\emptyset$ if $i\ne j$. In general,
  $i=1,\dots,N$, which means that $f$ is approximated by affine functions
  over $N$ regions. The piecewise affine approximation of $f$ can then be
  written as:
  \begin{equation}
    \label{eq:f_pwa}
    f_{pwa}\definedas f_a+f_{na}^i,~\text{for}~i~\text{such that}~(x,u)\in\set R^i.
  \end{equation}

  The big-$M$ formulation can be used to write \eqref{eq:f_pwa} in a form that
  is readily used in a mixed-integer program \cite{Schouwenaars2001}. To this
  end, let $M>0$ be a sufficiently large fixed scalar parameter, and let
  $z^i\in\{0,1\}$ be a binary variable indicating that $(x,u)\in\set R^i$ if and
  only if $z^i=1$. Then, the piecewise affine dynamics in mixed-integer
  programming form are encoded by the following set of constraints:
  \begin{subequations}
    \begin{align}
      \dot x &= f_a(t,x,u,g(u))+\inlinesum_{i=1}^{N} z^i f_{na}^i(t,x,u,g(u)), \\
      x &\ge \bar x^i+b_{L,x}^i-M(1-z^i), \\
      x &\le \bar x^i+b_{U,x}^i+M(1-z^i), \\
      u &\ge \bar u^i+b_{L,u}^i-M(1-z^i), \\
      u &\le \bar u^i+b_{U,u}^i+M(1-z^i), \\
      1 &= \inlinesum_{i=1}^N z^i.
    \end{align}
  \end{subequations}

\end{subsidebar}

\begin{subsidebar}

  \subsection{Nonlinear Rocket Landing}

  Consider the rocket dynamics in \eqref{eq:nonlinear_rocket_dynamics_accel}
  and, for simplicity, suppose that the mass is constant. Define the state
  $x\definedas (r,\dot r)\in\reals^6$ and the input
  $u\definedas T\in\reals^3$. The non-affine part of the dynamics
  \eqref{eq:f_decomposition} then takes the particular form:
  \begin{equation}
    \label{eq:nonlinear_rocket_f_na}
    f_{na}=\Matrix{
      0 \\
      g(r)-cm\inv\norm[2]{\dot r}\dot r
    }.
  \end{equation}

  For simplicity, let us consider only the nonlinear gravity term, $g(r)$. We
  will deal with atmospheric drag for AAV trajectory generation
  below. Suppose that $g(r)=(0,0,g_z(r_z))$, which means that we only need to
  consider the vertical component $g_z:\reals\to\reals$. A typical profile is
  $g_z(r_z)=-\mu/r_z^2$, where $\mu$ is the gravitational parameter. Given a
  reference point $\bar r_z^i$, we have:
  \begin{equation}
    \label{eq:g_z_i}
    g_z^i = g_z(\bar r_z^i)+g_z\der(\bar r_z^i)(r_z-\bar r_z).
  \end{equation}

  Using \eqref{eq:f_pwa} and \eqref{eq:g_z_i}, \figref{g_z_pwa_illustration}
  draws $g_{z,pwa}$.

\begin{csmfigure}[%
  position=H,
  caption={Illustration of a piecewise affine approximation of $g_z$, the
    $z$-component of the nonlinear gravity force, using
    \eqref{eq:g_z_i}.},
  label={g_z_pwa_illustration}]%
  \centering
  \centering
  \includegraphics[width=0.55\linewidth]{lcvx_g_z_pwa_illustration}
\end{csmfigure}

  \subsection{AAV Trajectory Generation Without Stalling}

  Consider the AAV dynamics in \eqref{eq:uav_dynamics} and, for simplicity,
  assume constant altitude flight. Define the state
  $x\definedas (r,v)\in\reals^4$ and the input $u=v_d\in\reals^2$. The
  non-affine part of the dynamics \eqref{eq:f_decomposition} then takes the
  particular form:
  \begin{equation}
    \label{eq:uav_f_na}
    f_{na}=\Matrix{
      0 \\
      -c\inv\norm[2]{v}v
    }.
  \end{equation}

  Let us focus on the aerodynamic drag term, $f_d=-c\norm[2]{v}v$. The first
  order Taylor expansion about a reference airspeed $\bar v^i$ is:
  \begin{equation}
    \label{eq:uav_f_d_i}
    f_d^i =
    -c\inv\|\bar v^i\|_2
    \brak[bigg]{I+\|\bar v^i\|_2^{-2}\bar v^i{\bar v^i}\T}
    (v-\bar v^i).
  \end{equation}

  Using \eqref{eq:f_pwa} and \eqref{eq:uav_f_d_i}, \figref{f_d_pwa_illustration}
  draws $f_{d,pwa}$. % Note that
  % the piecewise affine approximation can clearly be discontinuous across the
  % approximation validity region $\set R^i$ boundary.

\begin{csmfigure}[%
  position=H,
  caption={Illustration of a piecewise affine approximation of $f_{d_x}$,
    the $x$-component of the aerodynamic drag force, using
    \eqref{eq:uav_f_d_i}.},
  label={f_d_pwa_illustration}]%
  \centering
  \ifmaketwocolcsm
  \def\subfigwidth{0.55\linewidth}
  \else
  \def\subfigwidth{0.65\linewidth}
  \fi
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\subfigwidth]{lcvx_pwa_drag_continuous}
    \caption{Surface of the continuous function $-f_{d,x}$. The
      {\color{beamerBlue}blue} dots display operating points at which the
      gradient is evaluated.}
    \label{fig:lcvx_pwa_drag_continuous}
  \end{subfigure}%

  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\subfigwidth]{lcvx_pwa_drag_discrete}
    \caption{Surface of the discontinuous piecewise affine approximation
      $-f_{d_x,pwa}$. The {\color{beamerBlue}blue} dashed rectangle in the
      airspeed space shows the boundary of the approximation validity
      region $\set R^i$.}
    \label{fig:lcvx_pwa_drag_discrete}
  \end{subfigure}%
\end{csmfigure}

\end{subsidebar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

